Controlling Over-generalization and its Effect on Adversarial Examples Generation and Detection

Convolutional Neural Networks (CNNs) significantly improve the state-of-the-art for many applications, especially in computer vision. However, CNNs still suffer from a tendency to confidently classify out-distribution samples from unknown classes into pre-defined known classes. Further, they are also vulnerable to adversarial examples. We are relating these two issues through the tendency of CNNs to over-generalize for areas of the input space not covered well by the training set. We show that a CNN augmented with an extra output class can act as a simple yet effective end-to-end model for controlling over-generalization. As an appropriate training set for the extra class, we introduce two resources that are computationally efficient to obtain: a representative natural out-distribution set and interpolated in-distribution samples. To help select a representative natural out-distribution set among available ones, we propose a simple measurement to assess an out-distribution set's fitness. We also demonstrate that training such an augmented CNN with representative out-distribution natural datasets and some interpolated samples allows it to better handle a wide range of unseen out-distribution samples and black-box adversarial examples without training it on any adversaries. Finally, we show that generation of white-box adversarial attacks using our proposed augmented CNN can become harder, as the attack algorithms have to get around the rejection regions when generating actual adversaries.

==> Background.tex <==
\begin{figure}
    \centering
    \subfigure[MLP]{\includegraphics[width=0.2\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{Figures/in-dis}}
    \subfigure[Augmented MLP]{\includegraphics[width=0.2\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{Figures/out-learning_6}}
    \caption{Two-moons synthetic dataset.(a) MLP trained on only in-distribution samples (b) the augmented MLP trained on both in-distribution and some out-distribution samples }
\label{toyexample}
\end{figure}


\section{Preliminaries\label{sec:preliminaries}}
A Convolutional Neural Network (CNN) is constructed by a sequence of blocks, which each consists of convolution, ReLU and pooling layers, followed by a couple of fully connected layers. As the last layer, there is a softmax layer to translates the final fully connected layer outputs to class prediction. In other words, the output of a CNN is treated as a probability vector, where it comprises conditional probability of each class for a given input $x$. A CNN can be represented by function $Y=F(x,\theta)$ where $x\in[0,1]^{d}$ is an input image and $\theta$ represents its parameters (i.e. weights and biases).

%\hl{As previously discussed, despite their high accuracy, CNNs are susceptible to adversarial examples artificially generated using clean samples, with the aim of fooling} CNNs\cite{szegedy2013intriguing}. 

Generally, an adversarial generation method can either be targeted or untargeted. In targeted attacks, an adversary aims to generate an adversarial sample such that makes a victim CNN to misclassify it as a fooling target class(\ie~$\argmax F(x+\delta) = y'$, where $y'$ is the targeted class). 
%Formally speaking, an targeted attack explores for a smallest perturbation as follows: 
% \begin{equation}
% \begin{split}
% &\min_{\delta}\|\delta\|_p \\
% & \text{s.t} \quad \argmax \{F(x+\delta)\} = y' \quad \& \quad  x+\delta\in [0,1]^{d}
% \end{split}
% \end{equation}
% where $\|.\|_p$ is $L_p$ norm and $\delta$ is the perturbation (carefully learned noise) to be added to clean image $x$ such that the victim classifier $F$ misclassifies it as target class $y'$. 
In an untargeted attack, an adversary aims to make the victim CNN simply misclassifies it as some classes different than the true label (\ie~$\argmax F(x+\delta) \neq y^*$, where $y^*$ is the true class).
Here, we briefly explain some well-known targeted and untargeted attack algorithms.\\
\noindent\textbf{Targeted Fast Gradient Sign (T-FGS)~\cite{kurakin2016adversarial}:} This targeted attack method tends to modify a clean image $x$ so that the loss function is minimized for a given pair of $(x,y')$, where target class $y'$ is different from the input's true label ($y'\neq y^*)$. 
To this end, it uses the sign of gradient of loss function as follows: 
\begin{equation}
x_{adv}=x-\epsilon . sign(\nabla J(F(x,\theta),y')),
\end{equation}
 where $J(F(x,\theta),y')$ is the loss function and $\epsilon$ as the hyper-parameter controls the amount of distortion. The transferability of T-FGS samples increases by utilizing larger $\epsilon$ at the cost of adding more distortions to the image. Moreover, the untargeted variant of this method called FGS\cite{goodfellow2014explaining} is as follows:  
\begin{equation}
x_{adv}=x+\epsilon . sign(\nabla J(F(x,\theta),y^*)).
\end{equation}
\noindent\textbf{Iterative Fast Gradient Sign (I-FGS)~\cite{kurakin2017adversarial}:} This method actually is an iterative variant of Fast Gradient Sign, where iteratively small amount of FGS's perturbation is added by using a small value for $\epsilon$. To keep the perturbed sample in $~\alpha$-neighboring of $x$, the achieved adversary in each iteration should be clipped.
\begin{equation}
\begin{split}
& x_{adv}^{0}=x\\ & x_{adv}^{k+1}=\mathit{clip}_{x,\alpha}\{x_{adv}^{k}+\epsilon . sign(\nabla J(F(x_{adv}^{k},\theta),y^*))\},
\end{split}
\end{equation}
Compared to FGS, I-FGS generates more optimal distortions.

\noindent\textbf{DeepFool~\cite{moosavi2016deepfool}:} This algorithm is an iterative but fast approach for creation of untargeted attacks with very small amount of perturbations. Indeed, DeepFool generates sub-optimal perturbation for each sample where the perturbation is designed to transfer the clean sample across its nearest decision boundary.


\noindent\textbf{Carlini Attack (C\&W)~\cite{carlini2017towards}:} Unlike previous proposed methods which find the adversarial examples over loss functions of CNN, this method defines a different objective function which tends to optimize misclassification as follows:
\begin{equation}
f(x')=  \max(\max  \{Z(x')_{y'}}-Z(x')_{y^*} , -\kappa)
\end{equation}
Where $Z(x)$ is the output of last fully connected (before softmax layer) and $x'$ is perturbed image $x$.  Also $\kappa$ denotes  confidence parameter. The larger value for $\kappa$ leads the CNN to misclassify the input more confidently, while it leads  finding  adversarial examples satisfying the condition (having high miscalsification confidence) to be difficult.

\begin{figure}[t]
    \centering
    \subfigure{\includegraphics[width=0.4\textwidth]{Figures/interpolated_mnist_2}}
    \subfigure{\includegraphics[width=0.4\textwidth]{Figures/interpolated_cifar.pdf}}
    \caption{Interpolated samples for MNIST and CIFAR10. Third row represents the interpolated samples that are composed of images from first (source) and second rows (target).  }
    \label{fig:intimg}
    \vspace{-0.25in}
\end{figure}

\begin{comment}
if you would accept, i think this is more accurate for explaining carlini attack. Plus introducing some notations after the equation are redundant. So they can safely be removed
\begin{equation}
\begin{split}
    

&\min_{\delta}\|\delta\|_{p} +c .f(x)\\
&f(x)=  \max(\max  \{Y(x)_j: j\neq y^*\}-Y(x)_{y^*} , -\kappa)

\end{split}
\end{equation}


\end{comment}





==> ICLR 2019 Out-distribution (6)/Background.tex <==
\begin{figure}
    \centering
    \subfigure[MLP]{\includegraphics[width=0.2\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{Figures/in-dis}}
    \subfigure[Augmented MLP]{\includegraphics[width=0.2\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{Figures/out-learning_6}}
    \caption{Two-moons synthetic dataset.(a) MLP trained on only in-distribution samples (b) the augmented MLP trained on both in-distribution and some out-distribution samples }
\label{toyexample}
\end{figure}


\section{Preliminaries\label{sec:preliminaries}}
A Convolutional Neural Network (CNN) is constructed by a sequence of blocks, which each consists of convolution, ReLU and pooling layers, followed by a couple of fully connected layers. As the last layer, there is a softmax layer to translates the final fully connected layer outputs to class prediction. In other words, the output of a CNN is treated as a probability vector, where it comprises conditional probability of each class for a given input $x$. A CNN can be represented by function $Y=F(x,\theta)$ where $x\in[0,1]^{d}$ is an input image and $\theta$ represents its parameters (i.e. weights and biases).

%\hl{As previously discussed, despite their high accuracy, CNNs are susceptible to adversarial examples artificially generated using clean samples, with the aim of fooling} CNNs\cite{szegedy2013intriguing}. 

Generally, an adversarial generation method can either be targeted or untargeted. In targeted attacks, an adversary aims to generate an adversarial sample such that makes a victim CNN to misclassify it as a fooling target class(\ie~$\argmax F(x+\delta) = y'$, where $y'$ is the targeted class). 
%Formally speaking, an targeted attack explores for a smallest perturbation as follows: 
% \begin{equation}
% \begin{split}
% &\min_{\delta}\|\delta\|_p \\
% & \text{s.t} \quad \argmax \{F(x+\delta)\} = y' \quad \& \quad  x+\delta\in [0,1]^{d}
% \end{split}
% \end{equation}
% where $\|.\|_p$ is $L_p$ norm and $\delta$ is the perturbation (carefully learned noise) to be added to clean image $x$ such that the victim classifier $F$ misclassifies it as target class $y'$. 
In an untargeted attack, an adversary aims to make the victim CNN simply misclassifies it as some classes different than the true label (\ie~$\argmax F(x+\delta) \neq y^*$, where $y^*$ is the true class).
Here, we briefly explain some well-known targeted and untargeted attack algorithms.\\
\noindent\textbf{Targeted Fast Gradient Sign (T-FGS)~\cite{kurakin2016adversarial}:} This targeted attack method tends to modify a clean image $x$ so that the loss function is minimized for a given pair of $(x,y')$, where target class $y'$ is different from the input's true label ($y'\neq y^*)$. 
To this end, it uses the sign of gradient of loss function as follows: 
\begin{equation}
x_{adv}=x-\epsilon . sign(\nabla J(F(x,\theta),y')),
\end{equation}
 where $J(F(x,\theta),y')$ is the loss function and $\epsilon$ as the hyper-parameter controls the amount of distortion. The transferability of T-FGS samples increases by utilizing larger $\epsilon$ at the cost of adding more distortions to the image. Moreover, the untargeted variant of this method called FGS\cite{goodfellow2014explaining} is as follows:  
\begin{equation}
x_{adv}=x+\epsilon . sign(\nabla J(F(x,\theta),y^*)).
\end{equation}
\noindent\textbf{Iterative Fast Gradient Sign (I-FGS)~\cite{kurakin2017adversarial}:} This method actually is an iterative variant of Fast Gradient Sign, where iteratively small amount of FGS's perturbation is added by using a small value for $\epsilon$. To keep the perturbed sample in $~\alpha$-neighboring of $x$, the achieved adversary in each iteration should be clipped.
\begin{equation}
\begin{split}
& x_{adv}^{0}=x\\ & x_{adv}^{k+1}=\mathit{clip}_{x,\alpha}\{x_{adv}^{k}+\epsilon . sign(\nabla J(F(x_{adv}^{k},\theta),y^*))\},
\end{split}
\end{equation}
Compared to FGS, I-FGS generates more optimal distortions.

\noindent\textbf{DeepFool~\cite{moosavi2016deepfool}:} This algorithm is an iterative but fast approach for creation of untargeted attacks with very small amount of perturbations. Indeed, DeepFool generates sub-optimal perturbation for each sample where the perturbation is designed to transfer the clean sample across its nearest decision boundary.


\noindent\textbf{Carlini Attack (C\&W)~\cite{carlini2017towards}:} Unlike previous proposed methods which find the adversarial examples over loss functions of CNN, this method defines a different objective function which tends to optimize misclassification as follows:
\begin{equation}
f(x')=  \max(\max  \{Z(x')_{y'}}-Z(x')_{y^*} , -\kappa)
\end{equation}
Where $Z(x)$ is the output of last fully connected (before softmax layer) and $x'$ is perturbed image $x$.  Also $\kappa$ denotes  confidence parameter. The larger value for $\kappa$ leads the CNN to misclassify the input more confidently, while it leads  finding  adversarial examples satisfying the condition (having high miscalsification confidence) to be difficult.

\begin{figure}[t]
    \centering
    \subfigure{\includegraphics[width=0.4\textwidth]{Figures/interpolated_mnist_2}}
    \subfigure{\includegraphics[width=0.4\textwidth]{Figures/interpolated_cifar.pdf}}
    \caption{Interpolated samples for MNIST and CIFAR10. Third row represents the interpolated samples that are composed of images from first (source) and second rows (target).  }
    \label{fig:intimg}
    \vspace{-0.25in}
\end{figure}

\begin{comment}
if you would accept, i think this is more accurate for explaining carlini attack. Plus introducing some notations after the equation are redundant. So they can safely be removed
\begin{equation}
\begin{split}
    

&\min_{\delta}\|\delta\|_{p} +c .f(x)\\
&f(x)=  \max(\max  \{Y(x)_j: j\neq y^*\}-Y(x)_{y^*} , -\kappa)

\end{split}
\end{equation}


\end{comment}





==> ICLR 2019 Out-distribution (6)/Evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

We conduct several experiments on three benchmarks, namely MNIST, CIFAR-10, and CIFAR-100 datasets, using three neural network architectures LeNet~\citep{lecun1998gradient}, VGG-16~\citep{simonyan2014very}, and ResNet164~\citep{he2016identity}. To assess robustness of the augmented versions of these CNNs , we consider five well-known strong attack algorithms: Fast Gradient Sign (FGS)~\citep{goodfellow2014explaining}, Iterative FGS (I-FGS)~\citep{madry2017towards}, Targeted FGS (T-FGS)~\citep{kurakin2016adversarial}, DeepFool~\citep{moosavi2016deepfool}, and C\&W~\citep{carlini2017towards} (see Appendix~\ref{sec:advsettings} to learn about their hyper-parameter configurations). Note that we evaluate performance using three metrics: 1) accuracy (Acc.), which captures the rate or percentage of samples classified correctly as their true associated label; 2) rejection rate (Rej.), to measure the rate of samples correctly classified as dustbin (equivalent to rejection option); and 3) error rate (Err.), which captures the rate of samples that are neither correctly classified nor rejected.

%(30k randomly selected samples from the corresponding out-distribution set\footnote{As NotMNIST has only $\approx$18k samples in total, we used 10k (randomly selected) of them as training out-distribution samples, and the rest for testing.})
%1) classification of MNIST digits \cite{lecun1998mnist} with NotMNIST\footnote{Available at \url{http://yaroslavvb.blogspot.ca/2011/09/notmnist-dataset.html}.} printed letters as out-distribution dataset; 2) object recognition with CIFAR-10 as in-distribution dataset and a subset of unrelated classes from CIFAR-100 \cite{krizhevsky2009learning} as out-distribution samples; and 3) object recognition on CIFAR-100, with out-distribution samples taken from a subset of 62 classes of down-sampled ImageNet images \cite{chrabaszcz2017downsampled}. AlexNet \cite{krizhevsky2012imagenet} is used as classification model for the MNIST / NotMNIST setting, VGG-16 \cite{simonyan2014very} is used for CIFAR-10 / CIFAR-100, while ResNet-164 \cite{he2016identity} is the model for CIFAR-100 / ImageNet. More details on these datasets and experimental settings are provided in Sec.~\ref{sec:dataexp} of the Appendix. Experiments are done with five different well-known strong In the experiments, the error rates represents the percentage of wrong decisions made by CNNs for adversarial examples (\ie, when an adversarial example is neither rejected nor correctly classified). Experiments are conducted in a black-box setting (\ie attacks are generated using other models) and as well on white-box one (\ie attacks are generated using the target model).

\subsection{Black-box Adversarial Examples} 

It is widely known that many of adversarial examples generated from a learning model (e.g., CNN) can be transferred to attack other victim models~\citep{papernot2017practical,szegedy2013intriguing,carlini2017adversarial} --- such attacks are called \emph{transferable black-box attacks}. To evaluate robustness of the augmented CNNs on the aforementioned types of attacks generated in black-box setting, we generate adversarial samples corresponding to correctly classified clean test samples using a naive CNN, trained with different initial weights compared to the one under evaluation. 
Moreover, in order to demonstrate the influence of using different out-distribution sets for training the extra class on identifying adversaries, we employ four different sources for acquiring dustbin training samples:  1) adversarial samples generated by I-FGS; 2) only interpolated in-distribution data; 3) only a representative natural out-distribution set (selected according our proposed metric); and 4)  both interpolated samples along with a representative natural out-distribution set (selected according our proposed metric). 

To evaluate the generalization performance of the augmented CNNs on the in-distribution tasks, the in-distribution test accuracy rates are presented in Table~\ref{tab:blackboxresults}. Compared to the naive CNNs, we observe a slight drop in test accuracy rates of their augmented counterparts (except for that trained on I-FGS adversaries) while, interestingly, having also the error rates (i.e., the number of wrong decisions) reduced, leading to less error in decision making. This property can be highly beneficial for some security-sensitive applications, where making less error in some critical situations is vital.

\begin{table}[ht!]
\robustify\bfseries
\robustify\underline
\begin{scriptsize}
\begin{center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lll|S[table-format=3.2]|S[table-format=3.2]S[table-format=3.2]S[table-format=3.2]S[table-format=3.2]}
\toprule
&                &       &                          & \multicolumn{4}{c}{Augmented Models}\\
&                &       & {Naive Models}           & {Adversarial (I-FGS)}     & {Out-distribution}        & {Interpolation}           & {Out-dist. + Interp.}\\
\midrule
\multirow{19}{*}[0cm]{\begin{sideways}MNIST / NotMNIST (LeNet)\end{sideways}}
&                & Acc.  & 99.50                    & 99.54$^*$   & 99.47                     & 99.50                     & 99.48\\
& In-dist. (MNIST) test  & Rej. & {---}             & 0.00                      & 0.02                      & 0.02                      &  0.08\\
&                & Err.  & 0.50                     & 0.46                      & 0.51                      & 0.48                      & 0.44\\\cline{2-8}
& Out-dist. (NotMNIST) test & Rej.  & {---}         & 80.75                     & 99.96                     & 47.97                     & \bfseries{\num{99.98}}\\\cline{2-8}
&                & Acc.  & 35.14$^*$                & 0.00                      & 19.15                     & 10.47                     & 0.34\\
& FGS            & Rej.  & {---}                    & 100.00                    & 65.19                     & 83.31                     & 99.59\\
&                & Err.  & 65.86                    & \bfseries{\num{0.00}}     & 15.66                     & 6.22                      & 0.07\\\cline{2-8}
&                & Acc.  & 25.90                    & 0.00                      & 39.20$^*$                 & 3.10                      & 0.01\\
& I-FGS          & Rej.  & {---}                    & 100.00                    & 23.20                     & 95.69                     & 99.90\\
&                & Err.  & 74.10                    & \bfseries{\num{0.00}}     & 37.60                     & 1.21                      & 0.09\\\cline{2-8}
&                & Acc.  & 19.99$^*$                & 0.00                      & 1.17                      & 1.05                      & 0.00\\
& T-FGS          & Rej.  & {---}                    & 100.00                    & 95.92                     & 98.58                     & 100.00\\
&                & Err.  & 80.01                    & \bfseries{\num{0.00}}     & 0.37                      & \bfseries{\num{0.00}}     & \bfseries{\num{0.00}}\\\cline{2-8}
&                & Acc.  & 1.89                     & 6.21                      & 11.45$^*$                 & 9.87                      & 5.36\\
& DeepFool       & Rej.  & {---}                    & 35.66                     & 4.72                      & 78.06                     & 89.84\\
&                & Err.  & 98.11                    & 58.13                     & 83.83                     & 12.07                     & \bfseries{\num{4.80}}\\\cline{2-8}
&                & Acc.  & 22.49                    & 18.00                     & 27.50$^*$                 & 15.50                     & 7.50 \\
& C\&W ($L_2$)   & Rej.  & {---}                    & 28.00                     & 5.99                      & 55.00                     & 77.49\\
&                & Err.  & 77.51                    & 54.00                     & 66.51                     & 29.50                     & \bfseries{\num{15.01}}\\
\midrule
\midrule
\multirow{19}{*}[0cm]{\begin{sideways}CIFAR-10 / CIFAR-100$^{\dagger}$ (VGG)\end{sideways}}
&                & Acc.  & 90.53                    & 91.66$^*$                 & 88.58                     & 90.38                     & 86.65\\
& In-dist. (CIFAR-10) test  & Rej.  & {---}         & 0.10                      & 5.69                      & 1.55                      & 8.74 \\
&                & Err.  & 9.47                     & 8.24                      & 5.73                      & 8.07                      & \bfseries{\num{4.61}}\\\cline{2-8}
& Out-dist. (CIFAR-100$^{\dagger}$) test & Rej.  & {---}        & 0.82                      & 95.36                     & 5.00                      & \bfseries{\num{96.21}}\\\cline{2-8}
&                & Acc.  & 36.16                    & 0.00                      & 31.90                     & 38.98$^*$                 & 29.50\\
& FGS            & Rej.  & {---}                    & 100.00                    & 36.81                     & 6.93                      & 45.11\\
&                & Err.  & 63.84                    & \bfseries{\num{0.00}}     & 31.29                     & 54.09                     & 25.39\\\cline{2-8}
&                & Acc.  & 51.19                    & 0.00                      & 54.27                     & 59.22$^*$                 & 50.28\\
& I-FGS          & Rej.  & {---}                    & 100.00                    & 12.94                     & 5.06                      & 24.76\\
&                & Err.  & 48.81                    & \bfseries{\num{0.00}}     & 32.79                     & 35.72                     & 24.96\\\cline{2-8}
&                & Acc.  & 36.24$^*$                & 0.00                      & 27.17                     & 33.51                     & 24.35\\
& T-FGS          & Rej.  & {---}                    & 100.00                    & 41.08                     & 7.32                      & 51.33\\
&                & Err.  & 63.76                    & \bfseries{\num{0.00}}     & 31.75                     & 59.17                     & 24.32\\\cline{2-8}
&                & Acc.  & 56.82$^*$                & 46.52                     & 44.22                     & 54.48                     & 42.81\\
& DeepFool       & Rej.  & {---}                    & 14.12                     & 33.20                     & 5.16                      & 40.26\\
&                & Err.  & 43.18                    & 39.36                     & 22.58                     & 40.36                     & \bfseries{\num{16.93}}\\\cline{2-8}
&                & Acc.  & 42.50                    & 44.50                     & 46.50                     & 48.50$^*$                 & 39.00 \\
& C\&W ($L_2$)   & Rej.  & {---}                    & 1.50                      & 18.50                     & 8.00                      & 39.50\\
&                & Err.  & 57.50                    & 54.00                     & 35.00                     & 43.50                     & \bfseries{\num{21.50}}\\
\midrule
\midrule
\multirow{19}{*}[0cm]{\begin{sideways}CIFAR-100 / TinyImageNet$^{\dagger}$ (ResNet164)\end{sideways}}
&                & Acc.  & 75.52$^*$                & 75.33                     & 74.75                     & 73.68                     & 73.37\\
& In-dist. (CIFAR-100) test  & Rej.  & {---}        & 0.08                      & 0.93                      & 4.85                      & 5.02 \\
&                & Err.  & 24.48                    & 24.59                     & 24.32                     & 22.44                     & \bfseries{\num{21.61}}\\\cline{2-8}
& Out-dist. (TinyImageNet$^{\dagger}$) test & Rej.  & {---}         & 12.11                     & 97.24                     & 3.28                      & \bfseries{\num{97.33}}\\\cline{2-8}
&                & Acc.  & 67.67                    & 6.05                      & 50.15                     & 67.77$^*$                 & 50.03\\
& FGS            & Rej.  & {---}                    & 92.17                     & 34.22                     & 10.46                     & 36.87\\
&                & Err.  & 32.33                    & \bfseries{\num{1.78}}     & 15.63                     & 21.77                     & 13.10\\\cline{2-8}
&                & Acc.  & 22.20                    & 0.00                      & 16.90                     & 26.55$^*$                 & 16.80\\
& I-FGS          & Rej.  & {---}                    & 100.00                    & 32.65                     & 18.45                     & 45.75 \\
&                & Err.  & 77.80                    & \bfseries{\num{0.00}}     & 50.45                     & 55.00                     & 37.45\\\cline{2-8}
&                & Acc.  & 59.93$^*$                & 2.55                      & 37.87                     & 57.48                     & 37.07\\
& T-FGS          & Rej.  & {---}                    & 95.65                     & 44.12                     & 14.41                     & 46.87\\
&                & Err.  & 40.07                    & \bfseries{\num{1.80}}     & 11.76                     & 28.11                     & 16.06\\\cline{2-8}
&                & Acc.  & 77.20$^*$                & 73.77                     & 67.12                     & 73.02                     & 66.27\\
& DeepFool       & Rej.  & {---}                    & 0.95                      & 10.56                     & 5.85                      & 15.32\\
&                & Err.  & 22.80                    & 25.28                     & 22.32                     & 21.13                     & \bfseries{\num{18.41}}\\\cline{2-8}
&                & Acc.  & 74.50$^*$                & 68.00                     & 66.00                     & 68.00                     & 60.50\\
& C\&W ($L_2$ )  & Rej.  & {---}                    & 4.00                      & 16.50                     & 11.00                     & 25.50\\
&                & Err.  & 25.50                    & 28.00                     & 17.50                     & 22.00                     & \bfseries\num{14.00}\\
\bottomrule
\end{tabular}}
\end{center}
\end{scriptsize}
\caption{Results for black-box adversaries attacks on three classification tasks. Values with $^*$ denotes best accuracy while \textbf{boldface} denotes lowest misclassification rate for each given dataset and attack method.}
\label{tab:blackboxresults}
\vspace{-2.5\baselineskip}
\end{table}
 For the augmented CNNs, rejection rate (i.e., assignments to dustbin) is reported in addition to accuracy (i.e., correct classifications) and error rates (i.e., misclassifications)\footnote{From Table \ref{tab:blackboxresults} we can obtain out-distribution detection performance, with true positive rate as (in-distribution accuracy + error rate), false positive rate as (1 - out-distribution rejection rate), and false negative as in-distribution rejection rate. As the proposed approach is threshold-free, ROC curves and related measurements (e.g., AUC-ROC) are irrelevant.}. Comparing the augmented CNNs in Table~\ref{tab:blackboxresults} across different classification tasks, we can find that the augmented CNNs trained on a set of I-FGS adversaries can reject (classifying as dustbin) almost all test variants of FGS adversaries (i.e., FGS, I-FGS and T-FGS), however they fail to reject non-FGS variants of adversaries (e.g., C\&W and DeepFool), as well as the natural out-distribution sets (see Table~\ref{adv-augment} of Appendix~\ref{app1}). \textit{Accordingly, we emphasize that using the samples drawn from the vicinity of decision boundaries such as I-FGS adversaries as a single training source for the extra dustbin class of augmented CNN can not effectively control over-generalization}. 
 Contrary to I-FGS augmented CNN, augmented CNNs trained on a representative natural out-distribution set (selected according to our proposed metric) along with some interpolated samples consistently outperform their naive counterparts and the other augmented CNNs by achieving a drastic drop in error (misclassification) rates on all variants of adversaries,  even though these augmented CNNs are not trained on any specific type of adversaries. This illustrates that if an augmented CNN is trained on a representative out-distribution set along with  some interpolated samples, it can efficiently reduce over-generalization, resulting in generally well-performing model in the case of adversaries and various natural out-distribution samples. Due to space limitation, we place some results on the augmented CNNs trained with non-representative natural out-distribution sets in the Appendix~\ref{app1} in Table~\ref{cifar10SVHN} for illustrating the deficiency of such sets in controlling over-generalization.
 
 
To visualize and compare the classification regions in input space of our augmented CNN and its naive counterpart, we plot several church-windows (cross-sections)~\citep{warde201611} in Fig.~\ref{fig:church-win}. The x-axis of each window is the adversary direction achieved by FGS or DeepFool using the naive network. For each adversary direction, we plot four windows by taking four random directions that are perpendicular to the given adversary direction (x-axis). As it can be observed, the fooling classification regions (spanned by the adversary direction and one of its orthogonal random directions) of the naive CNNs are occupied by dustbin regions (indicated by orange) in their augmented counterparts. 

\begin{figure}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc}
\centering
&
\multicolumn{2}{c|}{MNIST} &
\multicolumn{2}{c}{CIFAR-10}\\
& Naive CNN & Augmented CNN & Naive VGG & Augmented VGG\\
\hline

&
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Naive_300.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Augment_300}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Naive_32.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Augment_32.pdf}}\\

%&
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Naive_482.pdf}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Augment_482}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Naive_700.pdf}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Augment_700.pdf}}\\

\multirow{5}{*}[1.75cm]{\begin{sideways}FGS\end{sideways}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Naive_539.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/FGS_CS_Augment_539}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Naive_386.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/FGS_CS_Augment_386.pdf}}\\
\hline
%&
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Naive_58.pdf}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Augment_58}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Naive_882.pdf}} &
%\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Augment_882.pdf}}\\
&
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Naive_351.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Augment_351}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Naive_389.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Augment_389.pdf}}\\
\multirow{5}{*}[1.75cm]{\begin{sideways}DeepFool\end{sideways}} & 
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Naive_828_s.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/mnist/selected/DeepFool_CS_Augment_828_s}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Naive_702.pdf}} &
\subfigure{\includegraphics[width=0.3\textwidth,trim=1cm 0.5cm 1cm 0.5cm,clip=true]{pics/cifar/selected/DeepFool_CS_Augment_702.pdf}}\\
\hline
&
\multicolumn{2}{m{0.6\textwidth}|}{\centering~~~~\includegraphics[height=0.92cm]{pics/mnist/colorbar_mnist_2.png}} &
\multicolumn{2}{m{0.6\textwidth}}{\centering~~\includegraphics[height=0.8cm]{pics/cifar/colorbar_cifar_2.png}}
\end{tabular}}
\caption{Church window plots for various data instances. Black dot corresponds to the clean sample position.}
\label{fig:church-win}
\vspace{-\baselineskip}
\end{figure}

\subsection{White-box Adversarial Examples}

White-box adversarial examples are generated by using directly the model on which they are applied. We further evaluate the robustness of our augmented CNNs on different types of white-box attacks, using the same parameter configurations as with the black-box experiments. For this purpose, we compute the percentage of visiting fooling classes (i.e., the classes different from dustbin and the true class associated to the clean samples) and the dustbin class when moving in the direction given by an attack method for a set of clean samples. Note that for generating some authentic white-box adversaries by the augmented CNNs, the attack algorithm should avoid dustbin regions to preclude generation of useless adversaries (those already recognizable as dustbin by the augmented CNN). In addition, the percentage of visiting the dustbin class when moving in a ``legitimate'' direction is also reported. By this we mean moving from a given sample $\mathbf{x}$ to its nearest neighbor $\mathbf{x}'$ from the \emph{same class} in the direction of their convex combination $(1-\epsilon)\,\mathbf{x}+\epsilon\,\mathbf{x}'$. Results for legitimate directions are computed with varying $\epsilon\in [0.1,0.5]$.

To generate white-box adversaries using both a naive CNN and its augmented counterpart, MNIST and CIFAR-10 test sets are utilized. As seen in Fig.~\ref{fig:barchartwhitebox}, adversaries generated for the augmented CNNs (trained on a representative natural out-distribution set) encounter more often the dustbin class than a fooling class, indicating that generation of white-box adversaries using the augmented CNNs becomes harder. An adversarial algorithm needs to skip over some regions assigned to dustbin class, leading to a possible increase in the number of steps or the amount of distortions required for generating adversaries. Moreover,  by moving in legitimate directions, the augmented CNNs appear to remain largely in the current true classes. 
\begin{figure}
\centering
\subfigure{\includegraphics[width=\textwidth,height=2.5cm]{pics/white-box.pdf}}
%\subfigure[MNIST]{\includegraphics[width=0.47\textwidth]{pics/cifar/mnist_Augm_CNN_diffDirections_ALL.pdf}}
%\subfigure[CIFAR-10]{\includegraphics[width=0.47\textwidth]{pics/cifar/cifar10_Augm_CNN_diffDirections_ALL.png}}
\caption{Robustness of naive CNNs (LeNet for MNIST (left) and VGG-16 for CIFAR-10 (right)) and their augmented counterparts under different adversarial attack algorithms. Robustness to white-box attacks is measured by the percentage of visiting fooling classes and dustbin class by moving in adversarial directions. }
\label{fig:barchartwhitebox}
%\vspace{-\baselineskip}
\end{figure}


\subsection{Out-distribution Samples}\label{sec:outdist}

The behavior of augmented CNNs is evaluated on several out-distribution sets across different in-distribution tasks.
 For each in-distribution dataset, we consider several natural out-distribution datasets, seen and unseen during the training of augmented CNNs. Table~\ref{tab:naturalOutDist} reports error and rejection rates for naive and the augmented CNNs (trained on a representative natural out-distribution set and interpolated samples). Note that the error rates for the augmented CNNs and their naive counterparts measure the number of the out-distribution samples classified with confidence higher than $50\%$ as one of the in-distribution classes. For further comparison, the rejection rates of two threshold-based approaches, including OpenMax~\citep{bendale2016towards} and Calibrated CNN~\citep{lee2017training}, are considered\footnote{The  code made available on Github by authors of those papers is used for our evaluation.}. These threshold-based approaches attempt to identify and reject out-distribution samples according to a specific optimal threshold on the calibrated predictive confidence scores. Likewise the authors~\citep{lee2017training}, the rejection rates for the Calibrated CNN and OpenMax are reported at true positive rate of $90\%$. 
 As can be seen in Table~\ref{tab:naturalOutDist}, the augmented CNN trained on a representative natural out-distribution set outperforms the two threshold-based approaches for CIFAR-10 and CIFAR-100 datasets. It should be noted that a Calibrated CNN can not converge during training for the datasets with a large number of classes such as CIFAR-100 (as in-dis. task), since this CNN is continuously forced to predict uniform confidence scores, which approach zero for large $K$ (i.e. number of classes), on the synthetic out-distribution samples. 
 %As it can be observed, while naive CNNs misclassify confidently most of out-distribution samples, their augmented counterparts reject them as dustbin with high confidence.
\begin{table}
\begin{center}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ll|S[table-format=3.2]|S[table-format=3.2]S[table-format=3.2]|c|c}
\hline
                            &                           & {Naive model} & \multicolumn{2}{c}{Augmented model}&OpenMax& Calibrated CNN\\ 
In-distribution train       & Out-distribution test     & {Error (\%)}  &  {Error (\%)} & {Rejection (\%)}& Rejection (\%)&Rejection (\%)  \\
\hline
\multirow{3}{*}{MNIST}      & NotMNIST (seen)           & 93.15         & 0.01          & 99.98 & 73.71&\textbf{100} \\
                            & Omniglot$^{*}$ (unseen)         & 95.19         & 0.00          & \textbf{100}&99.64 &\textbf{100}\\
                            & CIFAR-10(gc) (unseen) & 64.26        & 0.00          & \textbf{100}&90.35&99.8\\
\hline
\multirow{4}{*}{CIFAR-10}   & CIFAR-100$^{\dagger}$ (seen)    & 97.05         & 3.71          & \textbf{96.21}& 63.01&22.56\\
                            & TinyImageNet$^{\dagger}$ (unseen)   & 96.62         & 12.20         & \textbf{87.49}& 59.00&64.19\\
                            & SVHN (unseen)             & 95.56         & 7.61          & \textbf{92.29}& 45.37&25.32\\
                            & LSUN$^{*}$ (unseen)             & 96.12         & 14.31         & \textbf{84.80}& 68.34&72.81\\
\hline
\multirow{3}{*}{CIFAR-100}  & TinyImageNet$^{\dagger}$ (seen)     & 79.34         & 1.52          & \textbf{98.35}&67.30 & Nan\\
                            & SVHN (unseen)             & 81.19         & 67.75         & 16.25&\textbf{62.40}&Nan\\
                            & LSUN$^{*}$ (unseen)             &96.12       & 0.01          & \textbf{99.99}&73.23&Nan\\

\hline
\end{tabular}}
\end{center}
\caption{Comparison of augmented CNNs and threshold-based approaches on a range of natural out-distribution sets.  The size of input images of the datasets indicated by * are scaled to be consistent with their corresponding in-distribution set. CIFAR-10 (gc) means gray-scaled and cropped version of CIFAR-10.}
\label{tab:naturalOutDist}
\vspace{-\baselineskip}
\end{table}

\begin{comment}
\begin{table}[h!]
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|S[table-format=3.2]|S[table-format=3.2]}
\hline
\multirow{2}{*}{Dataset (in- / out-distribution)}& 
{Naive model error rate (\%)
$\downarrow$} &
{Augm. model rejection rate (\%)$\uparrow$}\\
 & 
{fooling samples from augm. model} &
{fooling samples from naive model}\\
\hline

MNIST / NotMINIST       & 88.79     & 95.49\\
CIFAR-10 / CIFAR-100    & 86.88     & 99.49\\
%CIFAR-100 / ImageNet    & \hl{xx}   & \hl{xx}\\
\hline
\end{tabular}}
\end{center}
\caption[Robustness of CNNs to transferability of rubbish fooling samples.]{Robustness of CNNs to transferability of rubbish fooling samples. Error rate of naive models corresponds to their misclassification with confidence over 50\,\%. The $\downarrow$ and $\uparrow$ indicate lower and upper values are better, respectively. }
\label{tab:foolingsamples}
\vspace{-\baselineskip}
\end{table}

Furthermore, it has also been shown that CNNs are also highly vulnerable to rubbish fooling samples~\cite{goodfellow2015explaining}, where each sample is initiated from some random noise, then using a classfier (CNN), some T-FGS perturbations are added to it iteratively until the underlying classifier misclassifies it into a selected target class. Using an augmented CNN and its naive counterpart, we generate two separate sets of fooling samples by T-FGS algorithm (see some fooling rubbish samples in Fig.~\ref{fig:rubbish_examples} in Appendix). Although one can still generate fooling rubbish samples from the augmented CNNs (in white-box setting), they can reject successfully the black-box fooling samples generated by a naive CNN. Therefore, most of the naive CNN's rubbish samples can be rejected by its augmented counterparts while the augmented CNN's rubbish samples can confidently fool a naive CNN (i.e., high misclassification rates) --- see Table~\ref{tab:foolingsamples}.
\end{comment}




\begin{comment}
\begin{figure}
\centering
\subfigure[MNIST, Naive CNN]{\includegraphics[width=0.475\textwidth]{pics/mnist/mnist_Naive_CNN_diffDirections_2.pdf}}
\subfigure[MNIST, Augmented CNN]{\includegraphics[width=0.475\textwidth]{pics/mnist/mnist_Augm_CNN_diffDirections_2.pdf}}\\
\subfigure[CIFAR-10, Naive VGG]{\includegraphics[width=0.475\textwidth]{pics/cifar/cifar10_Naive_CNN_diffDirections_2.pdf}}
\subfigure[CIFAR-10, Augmented VGG]{\includegraphics[width=0.475\textwidth]{pics/cifar/cifar10_Augm_CNN_diffDirections_2.pdf}}
\caption{Bar-charts of classification of samples generated by moving in directions of adversarial algorithms from a given initial clean sample. Legitimate consists in moving in direction of the same-class nearest neighbor. Each bar-chart is computed over XX initial clean samples, which a step size of YY in the adversarial directions \textbf{(CG: How about the step size for legitimate?)}.}
\label{fig:barchartwhitebox}
\end{figure}
\end{comment}


%In this section, a comprehensive evaluation is presented, where the augmented CNN is compared with a naive CNN on clean in-distribution samples as well as their adversaries that are generated by different first-order attack algorithms

% \begin{comment}
% \begin{table}[h]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l c|c|c|c|c|}
%     \hline
    
        
%          &&&&&&\\
%          \multicolumn{2}{|c|}{Training set: $<$in-dist, out-dist.$>$}&$<$MNIST, ---$>$&$<$MNIST, NotMNIST$>$&$<$MNIST, intrpl.$>$&$<$MNIST, NotMNIST+intrpl.$>$\\
%           &&&&&\\
%          \multicolumn{2}{|c|}{Model}&  Naive  CNN &Augmented CNN&Augmented CNN& Augmented CNN\\ \hline
         
%         In-dist. test& Acc.& \textbf{99.5}& 99.47 &99.38& 99.34  \\  \hline
        
%          Out-dist. test& Rej.&-& 99.96 &66.35&\textbf{99.98}\\  \hline
         
%       \multirow{3}{*}{FGS} & Acc& 35.14 & 19.15 &0.6 &0.58\\
%       &Rej&-&65.19&99.32&99.21\\ &Err& 65.86 & 15.66&0.08&\textbf{0.21}  \\
%       \hline
%         \multirow{3}{*}{I-FGS} & Acc& 25.90&39.2&0.5&0.7 \\
%         &Rej& -&23.2&99.5&99.3\\
%         &Err& 74.1&37.6&0.0&\textbf{0.0}\\ \hline
        
%         \multirow{3}{*}{T-FGS} & Acc& 19.99&1.17&0.04&0\\
%         &Rej&-&95.92&99.96&100\\ &Err& 80.01&2.91&0&\textbf{0}\\ \hline
        
%         \multirow{3}{*}{DeepFool}& Acc& 1.89&11.45&6.74&5.76\\
%         &Rej&-&4.72&86.90&85.89\\ &Err&98.11&83.83&\textbf{6.39}&8.44\\
%         \hline
%         \multirow{3}{*}{C\&W ($L_2$)} & Acc&22.49&27.5&7.0&8.0 \\ &Rej&-&5.99&80.0&79\\ &Err& 77.51&66.51&13&\textbf{13}\\ \hline
%         \hline
%         &&&&&\\
%         \multicolumn{2}{|c|}{Average Error rate}&79.106&40.94&&\\
%         &&&&&\\\hline
%     \end{tabular}}
%     \caption{Performance on black-box adversaries attacks. ``Acc.'' corresponds to accuracy (the rate of correctly classified samples), ``Rej.'' is the rejection rate, while ``Err.'' is the misclassification rate All results reported are percentages (\%).}
% \label{tab:mnist}
% \vspace{-0.2in}
% \end{table}
% \end{comment}


% \begin{table}[h!]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l c|c|c|c|c|}
%     \hline
    
        
%          &&&&&&\\
%          \multicolumn{2}{|c|}{Training set: $<$in-dist, out-dist.$>$}&$<$MNIST, ---$>$&$<$MNIST, NotMNIST$>$&$<$MNIST, intrpl.$>$&$<$MNIST, NotMNIST+intrpl.$>$\\
%           &&&&&\\
%          \multicolumn{2}{|c|}{Model}&  Naive  CNN &Augmented CNN&Augmented CNN& Augmented CNN\\ \hline
         
%         In-dist. test& Acc.& \textbf{99.5}& 99.47 &99.50& 99.48  \\  \hline
        
%          Out-dist. test& Rej.&-& 99.96 &47.97&\textbf{99.98}\\  \hline
         
%       \multirow{3}{*}{FGS} & Acc& 35.14 & 19.15 &10.47 &0.34\\
%       &Rej&-&65.19&83.31&99.59\\ &Err& 65.86 & 15.66&6.22&\textbf{0.07}  \\
%       \hline
%         \multirow{3}{*}{I-FGS} & Acc& 25.90&39.2&3.1&0.1 \\
%         &Rej& -&23.2&95.69&99.90\\
%         &Err& 74.1&37.6&1.21&\textbf{0.09}\\ \hline
        
%         \multirow{3}{*}{T-FGS} & Acc& 19.99&1.17&1.05&0\\
%         &Rej&-&95.92&98.58&100\\ &Err& 80.01&0.37&0&\textbf{0}\\ \hline
        
%         \multirow{3}{*}{DeepFool}& Acc& 1.89&11.45&9.87&5.36\\
%         &Rej&-&4.72&78.06&89.84\\ &Err&98.11&83.83&12.07&4.8\\
%         \hline
%         \multirow{3}{*}{C\&W ($L_2$)} & Acc&22.49&27.5&15.5&7.5 \\ &Rej&-&5.99&55&77.49\\ &Err& 77.51&66.51&29.5&\textbf{15.01}\\ \hline
%         \hline
%         &&&&&\\
%         \multicolumn{2}{|c|}{Average Error rate}&79.106&40.94&&\\
%         &&&&&\\\hline
%     \end{tabular}}
%     \caption{Performance on black-box adversaries attacks. ``Acc.'' corresponds to accuracy (the rate of correctly classified samples), ``Rej.'' is the rejection rate, while ``Err.'' is the misclassification rate All results reported are percentages (\%).}
% \label{tab:mnist}
% \vspace{-0.2in}
% \end{table}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table*}[h!]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l c|c|c| c|c|}
%     \hline

%          &&&&&&\\
%          \multicolumn{2}{|c|}{Training set: $<$in-dist, out-dist.$>$}&$<$CIFAR-10, ---$>$&$<$CIFAR-10, CIFAR100$>$&$<$CIFAR-10,intrpl.$>$&$<$CIFAR-10, CIFAR100+intrpl.$>$\\
%           &&&&&&\\
%          \multicolumn{2}{|c|}{Model}&   Naive  VGG &Augmented VGG&Augmented VGG&Augmented VGG\\ \hline
%         \multirow{3}{*}{In-dist. test}& Acc.&  \textbf{90.53}& 88.58&90.38& 86.65\\
%         &Rej&--&5.69&1.55&8.74\\
%         &Err&9.47&5.73&8.07&4.61\\
%         \hline
%          Out-dist. test& Rej.&-&95.36&5.0&\textbf{96.21}\\  \hline
%       \multirow{3}{*}{FGS} & Acc& 36.16&27.65&33.06&23.94\\ &Rej&-&38.94&7.5&49.28\\ 
%       &Err&63.84& 33.41&59.44&\textbf{25.11} \\
%       \hline
%         \multirow{3}{*}{I-FGS} & Acc&  51.19&47.6&50.60&43.2\\ 
%         &Rej& -&13.7&5.09&27\\
%         &Err& 48.81&39.33&44.31&\textbf{29.8}\\ \hline
%         \multirow{3}{*}{T-FGS} & Acc& 36.24&27.06&33.50&24.2\\ &Rej&-&40.54&7.5&50.69\\ &Err& 63.76&32.4&59&\textbf{24.84}\\ \hline
%         \multirow{3}{*}{DeepFool}& Acc&56.82&45.63&53.64&42.31\\ &Rej&-&30.75&5.41&38.76\\ &Err&43.18&23.9&40.95&\textbf{18.93}\\ \hline
%         \multirow{3}{*}{C\&W ($L_2$)} & Acc&42.5&46.5&48.50&39 \\ &Rej&-&18.5&8.0&39.5\\ &Err& 57.5&35&43.5&\textbf{21.5}\\ \hline
%         \hline
%         &&&&&\\
%         \multicolumn{2}{|c|}{Average Error} &55.41&32.80&49.44&\textbf{24.03}\\
%         &&&&&\\\hline
%     \end{tabular}}
%     \caption{Performance on black-box adversaries attacks. ``Acc.'' corresponds to accuracy (the rate of correctly classified samples), ``Rej.'' is the rejection rate, while ``Err.'' is the misclassification rate All results reported are percentages (\%).}
% \label{tab:cifar}
% \vspace{-0.2in}
% \end{table*}


%          &&&&&&\\
%          \multicolumn{2}{|c|}{Training set: $<$in-dist, out-dist.$>$}&$<$MNIST, ---$>$&$<$MNIST, NotMNIST$>$&$<$MNIST, intrpl.$>$&$<$MNIST, NotMNIST+intrpl.$>$\\
%           &&&&&\\
%          \multicolumn{2}{|c|}{Model}&  Naive  CNN &Augmented CNN&Augmented CNN& Augmented CNN\\ \hline
         
%         In-dist. test& Acc.& \textbf{99.5}& 99.47 &99.50& 99.48  \\  \hline
        
%          Out-dist. test& Rej.&-& 99.96 &47.97&\textbf{99.98}\\  \hline
         
%       \multirow{3}{*}{FGS} & Acc& 35.14 & 19.15 &10.47 &0.34\\
%       &Rej&-&65.19&83.31&99.59\\ &Err& 65.86 & 15.66&6.22&\textbf{0.07}  \\
%       \hline
%         \multirow{3}{*}{I-FGS} & Acc& 25.90&39.2&3.1&0.1 \\
%         &Rej& -&23.2&95.69&99.90\\
%         &Err& 74.1&37.6&1.21&\textbf{0.09}\\ \hline
        
%         \multirow{3}{*}{T-FGS} & Acc& 19.99&1.17&1.05&0\\
%         &Rej&-&95.92&98.58&100\\ &Err& 80.01&0.37&0&\textbf{0}\\ \hline
        
%         \multirow{3}{*}{DeepFool}& Acc& 1.89&11.45&9.87&5.36\\
%         &Rej&-&4.72&78.06&89.84\\ &Err&98.11&83.83&12.07&4.8\\
%         \hline
%         \multirow{3}{*}{C\&W ($L_2$)} & Acc&22.49&27.5&15.5&7.5 \\ &Rej&-&5.99&55&77.49\\ &Err& 77.51&66.51&29.5&\textbf{15.01}\\ \hline
%         \hline
%         &&&&&\\
%         \multicolumn{2}{|c|}{Average Error rate}&79.106&40.94&&\\
%         &&&&&\\\hline
%     \end{tabular}
%     \caption{Performance on black-box adversaries attacks. ``Acc.'' corresponds to accuracy (the rate of correctly classified samples), ``Rej.'' is the rejection rate, while ``Err.'' is the misclassification rate All results reported are percentages (\%).}
% \label{tab:mnist}
% \vspace{-0.2in}
% \end{table}




% \begin{table*}[h!]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l c|c|c| c|c|}
%     \hline

%          &&&&&&\\
%          \multicolumn{2}{|c|}{Training set: $<$in-dist, out-dist.$>$}&$<$CIFAR-100, ---$>$&$<$CIFAR-100, ImageNet$>$&$<$CIFAR-100,intrpl.$>$&$<$CIFAR-100, ImageNet+intrpl.$>$\\
%           &&&&&&\\
%          \multicolumn{2}{|c|}{Model}&   Resnet164 &Augmented VGG&Augmented VGG&Augmented VGG\\ \hline
%         \multirow{3}{*}{In-dist. test}& Acc.&  \textbf{69.2}& 68.15&66.02& 86.65\\
%         &Rej&--&0&5.07&8.74\\
%         &Err&30.8&31.85&29.91&4.61\\
%         \hline
%          Out-dist. test& Rej.&-&100&99.99&\textbf{96.21}\\  \hline
%       \multirow{3}{*}{FGS} & Acc& 36.16&27.65&33.06&23.94\\ &Rej&-&38.94&7.5&49.28\\ 
%       &Err&63.84& 33.41&59.44&\textbf{25.11} \\
%       \hline
%         \multirow{3}{*}{I-FGS} & Acc&  51.19&47.6&50.60&43.2\\ 
%         &Rej& -&13.7&5.09&27\\
%         &Err& 48.81&39.33&44.31&\textbf{29.8}\\ \hline
%         \multirow{3}{*}{T-FGS} & Acc& 36.24&27.06&33.50&24.2\\ &Rej&-&40.54&7.5&50.69\\ &Err& 63.76&32.4&59&\textbf{24.84}\\ \hline
%         \multirow{3}{*}{DeepFool}& Acc&56.82&45.63&53.64&42.31\\ &Rej&-&30.75&5.41&38.76\\ &Err&43.18&23.9&40.95&\textbf{18.93}\\ \hline
%         \multirow{3}{*}{C\&W ($L_2$)} & Acc&42.5&46.5&48.50&39 \\ &Rej&-&18.5&8.0&39.5\\ &Err& 57.5&35&43.5&\textbf{21.5}\\ \hline
%         \hline
%         &&&&&\\
%         \multicolumn{2}{|c|}{Average Error} &55.41&32.80&49.44&\textbf{24.03}\\
%         &&&&&\\\hline
%     \end{tabular}}
%     \caption{Should be updated.}
% \label{tab:cifar}
% \vspace{-0.2in}
% \end{table*}


% \begin{table}[h!]
%     \centering
%     \renewcommand{\arraystretch}{1}
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%     & \backslashbox{target}{source}&Naive CNN& Augmented-I&Augmented-II&Augmented-III\\
    
%         \multirow{3}{*}{MNIST}&Naive CNN (Err$\%$)&\cellcolor{blue!25}&85.53&&89.79\\
%         &Augmented-I (Rej$\%$)&100&\cellcolor{blue!25}&100&100\\
%         &Augmented-II (Rej$\%$)&63.5&1.60&\cellcolor{blue!25}&0\\
%         &Augmented-III (Rej$\%$)&95.49&100&100&\cellcolor{blue!25}\\
        
%         \hline
%         \multirow{3}{*}{CIFAR-10}&Naive CNN (Err$\%$)&\cellcolor{blue!25}&88.79&&86.88\\
%         &Augmented-I (Rej$\%$)&100&\cellcolor{blue!25}&100&100\\
%         &Augmented-II (Rej$\%$)&0&0&\cellcolor{blue!25}&0\\
%         &Augmented-III (Rej$\%$)&99.49&97.95&96.39&\cellcolor{blue!25}\\
%         \hline
%     \end{tabular}}
%     \caption{Assessment of robustness of CNNs on rubbish fooling samples. Augmented-I refers to an augmented-CNN trained only on natural out-distribution samples as class dustbin, "Augmented-II" is trained on only interpolated data as dustbin, and "Augmented-III" is trained on both interpolated and out-distribution samples as class dustbin.}
%     \label{tab:foolingsamples}
% \end{table}

% % Christian's version
% \begin{table}
% \robustify\bfseries
% \robustify\underline
% \centering
% \begin{tabular}{ll|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]}
% \hline
%                 &       &                           & \multicolumn{3}{c}{Augmented CNN}\\
%                 &       & {Naive CNN}               & {Out-distribution}        & {Interpolation}           & {Out-dist. + Interp.}\\\hline
%                 & Acc.  & \underline{\num{99.50}}   & 99.47                     & \underline{\num{99.50}}   & 99.48\\
% In-dist. test   & Rej.  & {---}                     & {xx}                      & {xx}                      & {xx}\\
%                 & Err.  & {xx}                      & {xx}                      & {xx}                      & {xx}\\\hline
% Out-dist. test  & Rej.  & {---}                     & 99.96                     & 47.97                     & \bfseries{\num{99.98}}\\\hline
%                 & Acc.  & \underline{\num{35.14}}   & 19.15                     & 10.47                     & 0.34\\
% FGS             & Rej.  & {---}                     & 65.19                     & 83.31                     & 99.59\\
%                 & Err.  & 65.86                     & 15.66                     & 6.22                      & \bfseries{\num{0.07}}\\\hline
%                 & Acc.  & 25.90                     & \underline{\num{39.20}}   & 3.10                      & 0.10\\
% I-FGS           & Rej.  & {---}                     & 23.20                     & 95.69                     & 99.90\\
%                 & Err.  & 74.10                     & 37.60                     & 1.21                      & \bfseries 0.09\\\hline
%                 & Acc.  & \underline{\num{19.99}}   & 1.17                      & 1.05                      & 0.00\\
% T-FGS           & Rej.  & {---}                     & 95.92                     & 98.58                     & 100.00\\
%                 & Err.  & 80.01                     & 0.37                      & 0.00                      & \bfseries 0.00\\\hline
%                 & Acc.  & 1.89                      & \underline{\num{11.45}}   & 9.87                      & 5.36\\
% DeepFool        & Rej.  & {---}                     & 4.72                      & 78.06                     & 89.84\\
%                 & Err.  & 98.11                     & 83.83                     & 12.07                     & \bfseries 4.80\\\hline
%                 & Acc.  & 22.49                     & \underline{\num{27.50}}   & 15.50                     & 7.50 \\
% C\&W ($L_2$)    & Rej.  & {---}                     & 5.99                      & 55.00                     & 77.49\\
%                 & Err.  & 77.51                     & 66.51                     & 29.50                     & \bfseries 15.01\\\hline
                    
% \end{tabular}
% \vspace{0.5em}
% \caption[Results for black-box adversaries attacks with MNIST dataset.]{Results for black-box adversaries attacks with MNIST dataset. Accuracy (``Acc.''), rejection rate (``Rej.'') and misclassification rate (``Err.'') are reported (percentages) for adversarial instances generated with Fast Gradient Sign (FGS), iterative FGS (I-FGS), targeted FGS (T-FGS), DeepFool and Carlini (C\&W) attacks. NotMNIST dataset has been used as source of out-distribution instances. \underline{Underline} denotes best accuracies while \textbf{boldface} denotes lowest misclassification rate for each given dataset and attack method.}
% \label{tab:mnist}
% \end{table}


% % Christian's version
% \begin{table}
% \centering
% \begin{tabular}{ll|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]}
% \hline
%                 &       &                           & \multicolumn{3}{c}{Augmented VGG}\\
%                 &       & {Naive VGG}               & {Out-distribution}        & {Interpolation}           & {Out-dist. + Interp.}\\\hline
%                 & Acc.  & \underline{\num{90.53}}   & 88.58                    & 90.38                      & 86.65\\
% % Acc.&  \textbf{90.53}& 88.58&90.38& 86.65\\
% In-dist. test   & Rej.  & {---}                     & 5.69                      & 1.55                      & 8.74 \\
% % &--&5.69&1.55&8.74\\
%                 & Err.  & 9.47                      & 5.73                      & 8.07                      & 4.61 \\\hline
% %         &Err&9.47&5.73&8.07&4.61\\
% Out-dist. test  & Rej.  & {---}                     & 95.36                     & 5.0                     & \bfseries\num{96.21}\\\hline
% % & Rej.&-&95.36&5.0&\textbf{96.21}\\  \hline
%                 & Acc.  & \underline{\num{36.16}}    & 27.65                    & 33.06                     & 23.94\\
% % & Acc& 36.16&27.65&33.06&23.94\\ &Rej&-&38.94&7.5&49.28\\
% FGS             & Rej.  & {---}                     & 38.94                     & 7.5                     & 49.28\\
% % &Rej&-&38.94&7.5&49.28\\ 
%                 & Err.  & 63.84                     & 33.41                     & 59.44                      & \bfseries\num{25.11}\\\hline
% %  &Err&63.84& 33.41&59.44&\textbf{25.11} \\
%                 & Acc.  & 51.19                     & 47.6                      & 50.60                      & 43.2\\
% % & Acc&  51.19&47.6&50.60&43.2\\
% I-FGS           & Rej.  & {---}                     & 13.7                     & 5.09                     & 27\\
% % &Rej& -&13.7&5.09&27\\
%                 & Err.  & 48.81                     & 39.33                     & 44.31                      & \bfseries\num{29.8}\\\hline
% %  &Err& 48.81&39.33&44.31&\textbf{29.8}\\ \hline
%                 & Acc.  & 36.24                     & 27.06                     & 33.50                      & 24.2\\
% % & Acc& 36.24&27.06&33.50&24.2\\
% T-FGS           & Rej.  & {---}                     & 40.54                     & 7.5                     & 50.69\\
% % &Rej&-&40.54&7.5&50.69\\
%                 & Err.  & 63.76                     & 32.4                      & 59                      & \bfseries\num{24.84}\\\hline
% %  &Err& 63.76&32.4&59&\textbf{24.84}\\
%                 & Acc.  & 56.82                      &45.63                      & 53.64                      & 42.31\\
% % Acc&56.82&45.63&53.64&42.31\\
% DeepFool        & Rej.  & {---}                     & 30.75                      & 5.41                     & 38.76\\
% % &Rej&-&30.75&5.41&38.76\\
%                 & Err.  & 43.18                     & 23.9                     & 40.95                     & \bfseries\num{18.93}\\\hline
% % &Err&43.18&23.9&40.95&\textbf{18.93}\\
%                 & Acc.  & 42.5                     & 46.5                      & 48.50                     & 39 \\
% % & Acc&42.5&46.5&48.50&39 \\
% C\&W ($L_2$)    & Rej.  & {---}                     & 18.5                      & 8.0                     & 39.5\\
% % &Rej&-&18.5&8.0&39.5\\
%                 & Err.  & 57.5                     & 35                     & 43.5                     & \bfseries\num{21.5}\\\hline
% % &Err& 57.5&35&43.5&\textbf{21.5}\\
% \end{tabular}
% \vspace{0.5em}
% \caption[Results for black-box adversaries attacks with CIFAR-10 dataset.]{Results for black-box adversaries attacks with CIFAR-10 dataset. Accuracy (``Acc.''), rejection rate (``Rej.'') and misclassification rate (``Err.'') are reported (percentages) for adversarial instances generated with Fast Gradient Sign (FGS), iterative FGS (I-FGS), targeted FGS (T-FGS), DeepFool and Carlini (C\&W) attacks. CIFAR-100 dataset has been used as source of out-distribution instances, using classes that are conceptually different from those of CIFAR-10. \underline{Underline} denotes best accuracies while \textbf{boldface} denotes lowest misclassification rate for each given dataset and attack method.}
% \label{tab:cifar10}
% \end{table}





% % Christian's version
% \begin{table}
% \centering
% \begin{tabular}{ll|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]|S[table-format=3.2]}
% \hline
%                 &       &                           & \multicolumn{3}{c}{Augmented ResNet164}\\
%                 &       & {Naive ResNet}               & {Out-distribution}        & {Interpolation}           & {Out-dist. + Interp.}\\\hline
%                 & Acc.  & \underline{\num{69.2}}   & 68.31                   & 66.27                      & 66.54\\
% % Acc.&  \textbf{90.53}& 88.58&90.38& 86.65\\
% In-dist. test   & Rej.  & {---}                     & 0.71                     & 4.85                      & 3.64 \\
% % &--&5.69&1.55&8.74\\
%                 & Err.  & 30.8                      & 30.98                      & 28.88                      & 29.82 \\\hline
% %         &Err&9.47&5.73&8.07&4.61\\
% Out-dist. test  & Rej.  & {---}                     & \bfseries\num{99.3  }                   & 4.4        &98.6  \\\hline
% % & Rej.&-&95.36&5.0&\textbf{96.21}\\  \hline
%                 & Acc.  & \underline{\num{36.16}}    & 27.65                    & 33.06                     & 23.94\\
% % & Acc& 36.16&27.65&33.06&23.94\\ &Rej&-&38.94&7.5&49.28\\
% FGS             & Rej.  & {---}                     & 38.94                     & 7.5                     & 49.28\\
% % &Rej&-&38.94&7.5&49.28\\ 
%                 & Err.  & 63.84                     & 33.41                     & 59.44                      & \bfseries\num{25.11}\\\hline
% %  &Err&63.84& 33.41&59.44&\textbf{25.11} \\
%                 & Acc.  & 31.3                     & 18.5                      & 27                     & 21.9\\
% % & Acc&  51.19&47.6&50.60&43.2\\
% I-FGS           & Rej.  & {---}                     & 36.2                     & 19.8                     & 36.2\\
% % &Rej& -&13.7&5.09&27\\
%                 & Err.  & 68.7                     & \bfseries\num{35.3 }      & 53.2                      & 41.9\\\hline
% %  &Err& 48.81&39.33&44.31&\textbf{29.8}\\ \hline
%                 & Acc.  & 22.6                     & 20.4                     & 19.91                      & 5.9\\
% % & Acc& 36.24&27.06&33.50&24.2\\
% T-FGS           & Rej.  & {---}                     & 63.9                     & 26.72                     & 84.95\\
% % &Rej&-&40.54&7.5&50.69\\
%                 & Err.  & 77.8                     & 15.7                      & 53.37                      & \bfseries\num{9.15}\\\hline
% %  &Err& 63.76&32.4&59&\textbf{24.84}\\
%                 & Acc.  & 77.2                      &75                      & 73.2                     & 71.9\\
% % Acc&56.82&45.63&53.64&42.31\\
% DeepFool        & Rej.  & {---}                     & 3                     & 5.6                    & 6.3\\
% % &Rej&-&30.75&5.41&38.76\\
%                 & Err.  & 22.8                     & 22                     & 21.2                     &21.9\\\hline
% % &Err&43.18&23.9&40.95&\textbf{18.93}\\
%                 & Acc.  & 77.5                     & 67                      & 68.50                     & 72.5 \\
% % & Acc&42.5&46.5&48.50&39 \\
% C\&W ($L_2$)    & Rej.  & {---}                     & 10                      & 10                     & 8.5\\
% % &Rej&-&18.5&8.0&39.5\\
%                 & Err.  & 22.5                     & 23                     & 21.5                     & \bfseries\num{19}\\\hline
% % &Err& 57.5&35&43.5&\textbf{21.5}\\

% \end{tabular}
% \vspace{0.5em}
% \caption[Results for black-box adversaries attacks with CIFAR-100 dataset.]{Results for black-box adversaries attacks with CIFAR-100 dataset. Accuracy (``Acc.''), rejection rate (``Rej.'') and misclassification rate (``Err.'') are reported (percentages) for adversarial instances generated with Fast Gradient Sign (FGS), iterative FGS (I-FGS), targeted FGS (T-FGS), DeepFool and Carlini (C\&W) attacks. CIFAR-100 dataset has been used as source of out-distribution instances, using classes that are conceptually different from those of CIFAR-10. \underline{Underline} denotes best accuracies while \textbf{boldface} denotes lowest misclassification rate for each given dataset and attack method.}
% \label{tab:cifar100}
% \end{table}


==> ICLR 2019 Out-distribution (6)/Intro.tex <==
\section{Introduction}
\label{sec:intro}


Convolutional Neural Networks (CNNs) have allowed for significant improvements over the state-of-the-art in the last few years for various applications, and in particular for computer vision. Notwithstanding these successes, challenging issues remain with these models. In the following work, we specifically look at two concerns. First, CNNs are vulnerable to different types of \emph{adversarial examples}  \citep{szegedy2013intriguing,kurakin2016adversarialb,moosavi2016deepfool,carlini2017towards}. These adversarial examples are created by deliberately modifying clean samples with imperceptible perturbations, with the aim of misleading CNNs into classifying them to a wrong class with high confidence. Second, CNNs are not able to handle instances coming from outside the task domain on which they are trained --- the so-called \emph{out-distribution samples}~\citep{liang2017principled,lakshminarayanan2017simple}. In other words, although these examples are semantically and statistically different from the (in-distribution) samples relevant to a given task, the neural network trained on the task assigns such out-of-concept samples with high-confidence to the pre-defined in-distribution classes. Due to the susceptibility of CNNs to both adversaries and out-distribution samples, deploying them for real-world applications, in particular for security-sensitive ones, is a serious concern.

%It has been shown that CNNs are highly vulnerable to various types of adversarial examples generated by a number of different attacks \citep{goodfellow2015explaining,kurakin2017adversarial,moosavi2016deepfool,papernot2017practical,carlini2017towards}.
 
These two issues have been treated separately in the past, with two distinct family of approaches. For instance, on the one hand, to handle out-distribution samples, some researchers have proposed threshold-based post-processing approaches with the aim of firstly calibrating the predictive confidence scores provided by either a single pre-trained CNN~\citep{liang2017principled,hendrycks2016baseline,lee2017training} or an ensemble of CNNs~\citep{lakshminarayanan2017simple}, and then detecting  out-distribution samples according to an optimal threshold. However, it is difficult to define an optimal and stable threshold for rejecting a wide range of out-distribution samples without increasing the false negative rate (i.e., rejecting in-distribution samples). On the other hand, researchers regarded adversarial examples as a distinct issue from the out-distribution problem and attempted to either correctly classify all adversaries through adversarial training of CNNs~\citep{tramer2017ensemble,goodfellow2015explaining,moosavi2016deepfool} or reject all of them by training a separate detector~\citep{feinman2017detecting,metzen2017detecting}. The performance of these approaches at properly handling adversarial instances mostly depends on having access to a diverse set of training adversaries, which is not only computationally expensive but also handling some possible future adversaries, which have not been discovered yet, most likely is difficult.

% what is my main idea?
%how measure contorlling of over-generalization:  which is measured here in term of the rejection rate of a broad-spectrum types of adversaries as well as natural out-distribution sets.
It is known that deep neural networks (e.g. CNNs) are prone to over-generalization in the input space by partitioning it \emph{entirely} into a set of pre-defined classes for a given in-distribution set (task), regardless of the fact that in-distribution samples may only be relevant to a small portion of the input space~\citep{liang2017principled,spigler2017denoising, bendale2016towards}. In this paper, we highlight that the two aforementioned issues of CNNs can be alleviated simultaneously through control of over-generalization. To this end,  we propose that an \emph{augmented CNN}, a regular (naive) CNN with an extra class dubbed as \emph{dustbin}, can be a simple yet effective solution, if it is trained on appropriate training samples for the dustbin class. Furthermore, we introduce here a computationally-efficient answer to the following key question: how to acquire such an appropriate set to effectively reduced the over-generalized regions induced by naive CNN. We note that our motivation for employing an augmented CNN is different from the threshold-based post-processing approaches that attempt to calibrate the predictive confidence scores of a pre-trained naive CNN without impacting its feature space. Our motivation in fact is to learn a
more expressive feature space, where along with learning the sub-manifolds corresponding to in-distribution classes, a distinct extra sub-manifold for the dustbin class can be obtained such that the samples
drawn from many over-generalized regions including a wide-range of out-distribution samples and various
types of adversaries are mapped to this ``dustbin'' sub-manifold.

%Through some extensive empirical evidences, we show that for augmented CNN properly trained on a representative set of out-distribution samples, over-generalized appears to be better controlling, with a better coverage of part of the input space associated out-distribution samples and adversaries.

%It should be mentioned that augmented CNNs previously have been employed for solely identifying adversaries~\citep{grosse2017statistical} by using a set of training adversarial examples for the extra class. Moreover, the authors did not aim at reducing over-generalization in order to classifying out-distribution samples as dustbin as well.to make an end-to-end learning model in order to capture a more expressive feature space through a distinct sub-manifold associated to the rejection option, in addition to the sub-manifolds corresponding to in-distribution classes.


%Note that ~\citet{lee2017training} have modified the generator's loss function of a GAN by adding a KL divergence term, forcing the predictive confidence scores of the synthetic samples obeys a uniform distribution. However, for large-scale datasets such as cifar100 or ImageNet, this term disappears as the uniform distribution becomes constant zero, leading to having an ordinary GAN for generating out-distribution samples.

% How to obtain 

As a training source for the extra class (dustbin), one can consider using synthetically generated out-distribution samples~\citep{lee2017training, jin2017introspective} or adversarial examples~\citep{grosse2017statistical}. However, using such generated samples is not only computationally expensive but also barely able to effectively reduce over-generalization compared to naive CNNs (see Sec.~\ref{sec:eval}). Instead of such synthetic samples, there are plenty of cost-effective training sources available for the extra dustbin class, namely \emph{natural out-distribution datasets}. By natural out-distribution sets we mean the sets containing some realitsic (not synthetically generated) samples that are semantically and statistically different from those in the in-distribution set. A \textit{representative} natural out-distribution set for a given in-distribution task should be able to adequately cover the over-generalized regions. To recognize such a representative natural set, we propose a simple measurement to assess its fitness for a given in-distribution set. In addition to the selected set, we  generate some artificial out-distribution samples through a straightforward and computationally efficient procedure, namely by interpolating some pair of in-distribution samples. We believe a properly trained augmented CNN can be utilized as a \emph{threshold-free baseline} for identifying concurrently a broad range of unseen out-distribution samples and different types of strong adversarial attacks. 
%and through extensive experiments on a range of different image datasets and varying CNNs, we demonstrate the reduction in over-generalization can reduce the misclassifcation rates on adversaries and out-distribution samples. We proceed by explicitly training augmented CNNs, which is augmented by an extra class named as "dustbin", on some natural and artificial-made  out-distribution samples (section.~\ref{sec:proposedmethod}) assigned the extra ``dustbin'' class. The main contributions of the paper are:
%By allowing a reject option for samples deemed irrelevant, we aim at limiting the effect of over-generalization. Experiments show that it limits the sensitivity of CNNs to adversarial and out-distribution samples. 


The main contributions of the paper are summarized as:
\begin{itemize}

% over-generalization as main idea of the paper
\item By \emph{limiting the over-generalization regions} induced by naive CNNs, we are able to drastically reduce the risk of misclassifying both adversaries and samples from a broad range of (unseen) out-distribution sets. To this end, we demonstrate that an \emph{augmented CNN} can act as a simple yet effective solution. 
\item We introduce a measurement to select a \emph{representative natural out-distribution set} among those available for training effective augmented CNNs, instead of synthesizing some dustbin samples using hard-to-train generators. 
%two enrich training source for the extra class of augmented CNN: 1) a representative natural out-distribution sets, , and 2) interpolated in-distribution samples. Moreover, these instances are key to achieve effective augmented CNNs, while being obtained with a relatively low computational burden when compared to approaches that generate samples.
% Moreover, these sources of dustbin examples can be obtained with a low computation burden, compared to generational approaches. 
%\item  with an additional dustbin class is . While it maintains in-distribution task accuracy rate when the dustbin class is trained on a \textit{representative} training set.

%As \textbf{natural out-distribution sets} are computationally lucrative sources for obtaining a \textit{representative} dustbin training set propose a metric to help with selecting  among the 
%We propose to train the augmented CNNs with natural out-distribution samples. We demonstrate that a simple metric relying on the distribution of misclassifications over the classes is a good indicator for selecting representative natural out-distribution sets to use for training over the dustbin class.

\item Based on extensive experiments on a range of different image classification tasks, we demonstrate that properly trained augmented CNNs can significantly reduce the misclassification rates for both 1)
\emph{unseen out-distribution sets}, and 2) for various types of \emph{strong black-box adversarial examples}, even though they are never trained on any specific types of adversaries.
%Through extensive experiments on a range of different vision tasks, we reveal We demonstrate experimentally the capacity for the augmented CNNs to limitover-generalization by our augmented CNNs can significant reduction in the misclassification rates on several out-distribution sets and robustness to several types of strong black-box adversarial examples. This is done using datasets and adversarial approaches not used during the training.

%\item We show that our augmented CNNs have the capacity to both \textbf{correctly classify} some of these adversaries (especially non-transferable ones) while \textbf{assigning the others to the dustbin class}, resulting in an overall reduction of misclassification rates. 
%(I am not sure about this claim)To our knowledge, such an approach has not been investigated by papers addressing adversarial samples or out-distribution samples.  

\item For the \emph{generation of white-box adversaries} using our proposed augmented CNN, the adversarial attack algorithms frequently encounter dustbin regions rather than regions from other classes when distorting a clean samples, making the adversaries generation process \emph{more difficult}.
%controlling over-generalization in the input space makes the \textit{creation of white-box} (i.e. adaptive) adversaries using a properly trained augmented CNN \textit{considerably more difficult} as the decision regions appear to be much more confined around the training samples.
%As many adversarial regions are successfully covered by dustbin regions, the attack algorithms should them to generate authentic adversaries.
%. It means that the amount of perturbation needed for generating adversaries should be increased in order to fool a properly trained augmented CNN. 


\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% commented out by Bobba on 9/27 at 9AM PT. See text above for replacement. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
The main contributions of the paper are summarized as:
\begin{itemize}

% over-generalization as main idea of the paper
\item We highlight that by \textbf{limiting the over-generalized regions} induced by a naive CNN, we can drastically reduce the risk of misclassifying both adversaries and  samples from a broad range of (unseen) out-distribution sets. To this end, we show that an augmented CNN trained on a representative training set for the extra class is a simple yet effective solution for controlling over-generalization, while it maintains the in-distribution test accuracy rate on its in-dist. task. 
% can be restricted by effectively limiting over-generalized regions induced by niave CNNs. To this end, an augmented CNN, as an end-to-end approach, is trained for learning an extra sub-manifold corresponding to the dustbin class.
%in order to automatically map \emph{a wide-range of unseen out-distribution samples and many of adversaries on it}. This causes the problem-relevant samples are untangled from them in this new feature space while they are fused or in close proximity of each other in the naive CNNs' feature space.

%\item We show a \emph{properly trained augmented CNN} as a baseline approach for controlling over-generalization, is enabled to identify (i.e. classifying as dustbin) a wide range of \textit{unseen} out-distribution samples as well as rubbish fooling samples (\ie meaningless samples like random noise confidently fooling naive CNNs). Meanwhile its accuracy on in-distribution sets is maintained.

% a metric
\item 
\textit{Natural out-distribution sets} are computationally lucrative training source for the extra class of augmented CNNs. For that purpose, we propose a metric for selecting a representative natural out-distribution set among the possible candidates for a given in-distribution task.
%We propose to train the augmented CNNs with natural out-distribution samples. We demonstrate that a simple metric relying on the distribution of misclassifications over the classes is a good indicator for selecting representative natural out-distribution sets to use for training over the dustbin class.

\item Through extensive experiments on a range of different vision tasks, we demonstrate the augmented CNNs trained on a single natural out-distribution set can significantly reduce the misclassification rates of the
\textbf{unseen out-distribution sets} and varying types of \textbf{strong black-box adversarial examples} while
they are never trained on any specific types of adversaries.
%Through extensive experiments on a range of different vision tasks, we reveal We demonstrate experimentally the capacity for the augmented CNNs to limitover-generalization by our augmented CNNs can significant reduction in the misclassification rates on several out-distribution sets and robustness to several types of strong black-box adversarial examples. This is done using datasets and adversarial approaches not used during the training.

\item We show that our augmented CNNs have the capacity to both \textbf{correctly classify} some of these adversaries (especially non-transferable ones) while \textbf{assigning the others to the dustbin class}, resulting in an overall reduction of misclassification rates. 
%(I am not sure about this claim)To our knowledge, such an approach has not been investigated by papers addressing adversarial samples or out-distribution samples.  

\item We also demonstrate that controlling over-generalization in input space makes the \textbf{creation of white-box} (i.e. adaptive) adversaries using a properly trained augmented CNN \textbf{considerably more difficult}. As many adversarial regions are successfully covered by dustbin regions, the attack algorithms should cross them to generate authentic adversaries.
%. It means that the amount of perturbation needed for generating adversaries should be increased in order to fool a properly trained augmented CNN. 


\end{itemize}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% commented out by Bobba on 9/27 at 9AM PT. See text above for replacement. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
\begin{figure}
\centering
\subfigure[In-distribution training only]{\includegraphics[width=0.35\textwidth]{Figures/toyexamplePre.pdf}}
\hspace*{2em}
\subfigure[In- and out-distribution training]{\includegraphics[width=0.45\textwidth]{Figures/toyexamplePost.pdf}}
\caption{Input space plot of a 2D illustrative problem: (a) classification with only in-distribution training, where regions 1, 3, 5, and 7 can be classified with high confidence to an arbitrary class; and (b) classification with in- and out-distribution training, only region 3 can be assigned to an arbitrary class, regions 1, 5, and 7 being assigned to the dustbin label (reject).}
\label{fig:toyexample}
\end{figure}
\end{comment}


==> ICLR 2019 Out-distribution (6)/ProposedMethod.tex <==


%(a) MLP trained on two classes classifies the space into two classes even some regions are not related to in-distribution regions. Therefore, this MLP is prone to over-generalization on these vacant regions that belong to out-distribution; (b) the augmented MLP trained on both in-distribution and some out-distribution samples can alleviate over-generalization in some out-distribution regions.



% \begin{figure*}

% %\resizebox{\textwidth}{!}{

% \begin{tabular}{>{\centering\arraybackslash}M{0.5cm}>{\centering\arraybackslash}m{0.5cm}>{\centering\arraybackslash}m{6cm}>{\centering\arraybackslash}m{6cm}>{\centering\arraybackslash}m{6cm}>{\centering\arraybackslash}}
% \centering

% && Clean~\&out-dist.& FGS & T-FGS \\

% \multirow{2}{*}{\parbox{1\linewidth}{\vspace{1.6cm} \rotatebox[origin=c]{90}{MNIST}}}&\rotatebox[origin=c]{90}{Naive CNN}  & \subfigure{\includegraphics[width=0.2\textwidth,trim=10cm 10cm 2cm 10cm, clip=true]{Figures/mnist_outdist_CNN.pdf}}& \subfigure{\includegraphics[width=0.2\textwidth,trim=9cm 10cm 2cm 10cm, clip=true]{Figures/mnist_FGS_CNN.pdf}}&\subfigure{\includegraphics[width=0.2\textwidth,trim=10cm 10cm 2cm 10cm, clip=true]{Figures/mnist_TFGS_CNN.pdf}}\\
% &\rotatebox[origin=c]{90}{Augmented CNN} & \subfigure{\includegraphics[width=0.22\textwidth,trim=10cm 10cm 4cm 10cm, clip=true]{Figures/Dustbin_CNNDust.pdf}}
% &\subfigure{\includegraphics[width=0.22\textwidth,trim=10cm 10cm 4cm 10cm, clip=true]{Figures/FGS_CNNDust-main.pdf}}
% &\subfigure{\includegraphics[width=0.22\textwidth,trim=10cm 10cm 4cm 10cm, clip=true]{Figures/TFGS_CNNDust.pdf}}\\ \hline
% \multirow{2}{*}{\parbox{1\linewidth}{\vspace{2cm} \rotatebox[origin=c]{90}{CIFAR-10}}}
% &   \rotatebox[origin=c]{90}{Naive VGG}  & \subfigure{\includegraphics[width=0.2\textwidth,trim=7cm 7cm 3cm 6cm, clip=true]{Figures/cifar_out_CNN}}  & \subfigure{\includegraphics[width=0.2\textwidth,trim=7cm 7cm 3cm 6cm, clip=true]{Figures/cifar_FGS_CNN}}     &\subfigure{\includegraphics[width=0.2\textwidth,trim=7cm 7cm 3cm 6cm, clip=true]{Figures/cifar_TFGS_CNN}}\\
% &\rotatebox[origin=c]{90}{ugmented VGG} & \subfigure{\includegraphics[width=0.2\textwidth,trim=4cm 5cm 4cm 6cm, clip=true]{Figures/cifar_out_CNNDust}}
% &\subfigure{\includegraphics[width=0.2\textwidth,trim=4cm 5cm 4cm 6cm, clip=true]{Figures/cifar_FGS_CNNDust}}
% &\subfigure{\includegraphics[width=0.2\textwidth,trim=7cm 5cm 4cm 6cm, clip=true]{Figures/cifar_TFGS_CNNDust}}
% \end{tabular}
% %}
% \caption{Visualization of some randomly selected test samples and their corresponding adversaries (FGS and T-FGS) in the feature spaces (the penultimate layer) learned by a naive CNN and an augmented CNN. To produce and manipulate the 3D plots refer to~ \url{https://github.com/mahdaneh/Out-distribution-learning_FSvisulization}}
% \label{fig:PCA-LCONV}
% \vspace{-0.20in}
% \end{figure*}



\section{Proposed Method}
\label{sec:proposedmethod}
%\subsection{Overview}
The key idea of this paper is to make use of a CNN augmented with a dustbin class, trained on a representative set of out-distribution samples, as a simple yet effective candidate solution to limit over-generalization. A visual illustration of this is given in Fig.~\ref{toyexample}, which provides a schematic explanation of the influence of training samples used to learn the dustbin class on the out-distribution area coverage. 
\begin{figure}[t]
   \centering
    \subfigure[{Naive MLP}]{\includegraphics[width=0.23\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{pics/in-dis.pdf}}~~
    \subfigure[{Dustbin samples draw around the decision boundary}]{\includegraphics[width=0.23\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{pics/onBoundry-learning_8.pdf}}~~
    \subfigure[{Non-representative set of dustbin samples}]{\includegraphics[width=0.23\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{pics/not-well-distributed-learning_8.pdf}}~~
    \subfigure[{Representative set of dustbin samples}]{\includegraphics[width=0.23\textwidth, trim= 1cm 0cm 1cm 1cm, clip=true]{pics/our-learning_5.pdf}}
    \caption{Illustration of the influence of different sets of dustbin training samples on the over-generalized regions. Two-moon classification dataset: (a) naive MLP trained only with in-distribution samples, (b-d) augmented MLPs trained with different out-distribution sets as dustbin. The MLP is made of three layers and ReLU activation functions.}
 \label{toyexample}
  \vspace{-\baselineskip}
 \end{figure}


This figure illustrates how the choice of training samples for the extra dustbin class plays a central role for achieving an effective augmented CNN. With a naive MLP (no dustbin class), a decision boundary is separating the whole input space into two classes (Fig.~\ref{toyexample}(a)), working on the complete input space even in regions that are deemed irrelevant for the task at hand. As for augmented MLPs, the second plot (Fig.~\ref{toyexample}(b)) shows results with dustbin training samples picked to be around the decision boundary, where many adversarial examples~\citep{moosavi2016deepfool} are designed to be located. As it can be observed, such augmented MLP can only slightly reduce over-generalized regions. However, it
might be able to classify some of adversaries as dustbin, and make generation of new adversaries
harder since the adversarial attack algorithm should avoid the dustbin regions that are now located in
between the two in-distribution classes. Thus, using solely such adversaries as training set of the dustbin class can not adequately cover the over-generalized regions. In another variation (Fig.~\ref{toyexample}(c)), the dustbin samples come from a out-distribution set, quite compact and located around the in-distribution samples from one specific class. Training an augmented MLP on this kind of out-distribution samples cannot reduce over-generalization effectively. Accordingly, we argue that out-distribution training samples that are distributed uniformly w.r.t in-distribution classes can be regarded as \emph{a representative set} for the extra dustbin class (Fig.~\ref{toyexample}(d)). Indeed, an augmented MLP trained on a representative set is able to classify a wide-range of unseen out-distribution sets and some of adversaries as its extra class, being more effective at controlling over-generalization. It is worth to note that coupling a representative out-distribution set with the samples drawn around the decision boundaries can further strengthen the augmented neural network against adversarial examples.

There are many possible ways of acquiring some training samples for the extra class of augmented CNNs, ranging from artificially generated samples~\citep{jin2017introspective,lee2017training} to natural available out-distribution sets. Instead of making use of a generator, which is computationally expensive and hard to train, we propose the use of two cost-effective resources for acquiring dustbin training samples in order to train effective augmented CNNs: i) a selected representative natural out-distribution set and ii) interpolated samples.

\subsection{Natural out-distribution instances}

A possible rich and readily accessible source of dustbin examples for training augmented models lies in natural out-distribution datasets. These sets contain natural samples that are statistically and semantically different compared to the samples of a given task. For example, NotMNIST and Omniglot datasets can be regarded as natural out-distribution sets when trying to classify MNIST digits. However, it is not clear how to select a sufficiently representative set from the (possibly large) corpus of available datasets in order to properly train augmented CNNs. We shed light on the selection of a representative \emph{natural out-distribution set} by introducing a simple visualization metric. Specifically, we deem a natural out-distribution set as representative for a given in-distribution task if it is misclassified uniformly over the in-distribution classes. That is, if roughly an equal number of out-distribution samples are classified confidently as belonging to each of the in-distribution classes by the naive neural network. 
Accordingly, to assess the appropriateness of out-distribution sets for a given task (or in-distribution set), we visualize the number of out-distribution samples that are misclassified to each of the in-distribution classes by using a histogram. In other words, a natural out-distribution set which has a more uniform misclassification distribution over the in-distribution classes appears better suited for training an effective augmented CNN.

In Fig.~\ref{fig:misclassify_uniform}, the uniformity characteristics of SVHN vs CIFAR-100$^\dagger$ as out-distribution sets for CIFAR-10, and LSUN vs TinyImageNet$^{\dagger}$ for CIFAR-100 are shown\footnote{Throughout the paper, $\dagger$ indicates a modified out-distribution set by discarding the classes that have exact or semantic overlaps with the classes of its corresponding in-distribution set. For example, the super-classes of vehicle from CIFAR-100 is removed due to their semantic overlap with automobile and truck classes of CIFAR-10. Refer to Appendix~\ref{app1} for detail information. }. According to Fig.~\ref{fig:misclassify_uniform}(a), most of SVHN samples are misclassified into a limited number of CIFAR-10 classes (5 classes out of 10 classes), while CIFAR-100$^{\dagger}$ exhibits a relatively more uniform misclassifcation on CIFAR-10 classes. Therefore, compared with SVHN, we consider CIFAR-100 as a more representative natural out-distribution set for CIFAR-10. A full comparison of these two out-distribution sets according to their ability to control over-generalization can be found in Table~\ref{cifar10SVHN} of the Appendix. Similar behaviour can also be observed for LSUN vs TinyImageNet as two out-distribution resources for training an augmented Resnet164 on CIFAR-100 (as in-distribution). In this case TinyImageNet$^{\dagger}$ has a more uniform distribution when compared with LSUN. 
\begin{figure}
\centering
\subfigure[CIFAR100$^{\dagger}$ (left) vs SVHN (right) for CIFAR-10]{\includegraphics[width=\textwidth]{pics/cifar100vsSVHN}}
\subfigure[TinyImageNet$^{\dagger}$ (left) vs LSUN (right) for CIFAR-100]{\includegraphics[width=\textwidth]{pics/cifar100_ImageNet}}
\caption{Misclassification distribution over original classes: (a) CIFAR-100$^{\dagger}$ vs SVHN provided by a naive VGG trained on CIFAR-10; (b) TinyImageNet$^{\dagger}$ vs LSUN provided by a naive Resnet-164 trained on CIFAR-100.}
    \label{fig:misclassify_uniform}
    \vspace{-\baselineskip}
\end{figure}
%In~\citep{tramer2017space}, the authors have shown a kind of interpolated data for MNIST as model-agnostic attacks to linear classifiers

\subsection{Interpolated instances} 

Algorithms to generate adversarial examples tend to produce results near (on margin) decision boundaries separating two classes~\citep{moosavi2015deepfool}. Adding a set of diverse types of adversaries to a representative natural out-distribution set may further improve the rate of adversary identification by the augmented CNN. But generating such a diverse set of adversarial examples for large-scale datasets is computationally expensive. Furthermore, using only adversaries as dustbin training samples (without including a representative natural out-distribution set) cannot lead to an effective reduction of over-generalization (see Fig.~\ref{toyexample}(b) and results in Sec.~\ref{sec:eval}).

Instead of generating adversarial examples for training, we propose an inexpensive and straightforward procedure for acquiring some samples around the decision boundaries. To this end, we interpolate some pairs of correctly classified in-distribution samples from different classes.  An interpolated sample created from two samples with different classes aims to cover such regions (margins around decision boundaries) between two classes in order to assign them to out-distribution (dustbin) regions. 
%and $H_{\theta}=F_\theta^1(G_\theta^0)$ as a classifier (CNN), where  $G_\theta^0$ is the feature extractor (the last convolutional layer), and $F_\theta^1$ is its classifier part.
Formally speaking, consider a pair of input images from two different classes of a K-classification problem, i.e. $\mathbf{x}_i, \mathbf{x}_j\in\mathbb{R}^{D}$  $i,j\in\{1,...,K\}$, where $\mathbf{x}_j$ is the nearest neighbor of $\mathbf{x}_i$ in the feature space of a CNN (its last convolution layer).  An interpolated sample $\mathbf{x}'\in R^{D}$ is generated by making a linear combination of the given pair in the input space, $\mathbf{x}'= \alpha\, \mathbf{x}_i + (1-\alpha)\, \mathbf{x}_j$. For all our experiments, we set $\alpha=0.5$. Some interpolated samples can be seen in Fig.~\ref{fig:interpolated} for MNIST and CIFAR-10. The reasons for finding the nearest neighbors in the feature space are twofold: computationally less expensive yet more accurate~\citep{bengio2009learning} when compared to doing so in high-dimensional input space.
\begin{figure}
\centering
\subfigure[CIFAR10 interpolation]{\includegraphics[width=0.475\linewidth]{pics/interpolated_cifar.pdf}}
\subfigure[MNIST interpolation]{\includegraphics[width=0.475\linewidth]{pics/interpolated_mnist.pdf}}
\caption{Interpolated samples for CIFAR10 and MNIST. Third row for every dataset represents the interpolated samples that are composed of images from first (source) and second rows (target).}
\label{fig:interpolated}
\vspace{-\baselineskip}
\end{figure}


 %With interpolation, we expose the network to images with mixed features from different classes, with associated target decision to reject them (assign to dustbin).
 % We aim at  The rationale behind the method is that an adversarial example contains the relevant features from two (or more) classes (i.e., true class and the target fooling class), where the features of the target fooling class are hardly visible while the features related to the true class can be recognizable for human observers.t


\subsection{Feature space of augmented CNNs}

As an augmented CNN is trained in a end-to-end fashion, it allows learning of an extra sub-manifold corresponding to the added extra class (dustbin). Thus, if the augmented CNN is trained properly on a representative out-distribution set, it is able to map a large variety of out-distribution sets onto its extra sub-manifold, whether or not they have been seen during training. This should allow to learn a feature space that untangles the in-distribution set from the out-distribution samples. This is in contrast to the feature space of its naive counterpart, where the in-distribution and out-distribution samples are likely to be mixed or placed near each other. 

Moreover, a proper trained augmented CNN is surprisingly able to map a large portion of black-box adversaries onto its extra manifold, even though it is never trained on any adversaries. Meanwhile some of the adversarial instances are mapped to their corresponding true class' sub-manifold. Therefore, this leads to a more engaging classifier for many practical situations (real-world applications) as some of adversaries are classified into dustbin (equivalent to the rejection option) while some of remaining ones are correctly classified as their true class (particularly non-transferable adversaries attacks, see Sec.\ref{sec:eval}).


In Fig.~\ref{fig:PCA-LCONV}, we exhibit the feature spaces achieved from a naive CNN and its augmented counterpart for CIFAR-10 as an in-distribution task.
\begin{figure}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|cc}
\multicolumn{2}{c|}{Naive CNN}&\multicolumn{2}{c}{Augmented CNN}\\
\subfigure{\includegraphics[width=0.20\textwidth,trim=7cm 7cm 3cm 6cm, clip=true]{Figures/cifar_out_CNN}} &
\subfigure{\includegraphics[width=0.20\textwidth,trim=7cm 7cm 3cm 6cm, clip=true]{Figures/cifar_FGS_CNN}} &
\subfigure{\includegraphics[width=0.20\textwidth,trim=4cm 5cm 4cm 6cm, clip=true]{Figures/cifar_out_CNNDust}}&
\subfigure{\includegraphics[width=0.20\textwidth,trim=4cm 5cm 4cm 6cm, clip=true]{Figures/cifar_FGS_CNNDust}}
\end{tabular}}
\caption{Visualization of data distribution in last convolution layer (i.e., feature space) of an augmented CNN trained on CIFAR-10 and CIFAR-100 as in-distribution and out-distribution sets, respectively. For visualization purposes, these feature spaces are reduced to 3D using PCA. For more results, refer to Fig~\ref{fig:PCA-LCONV2} of the Appendix.}
\label{fig:PCA-LCONV}
%\vspace{-\baselineskip}
\end{figure}
Note CIFAR-100 is used as the training set for the extra class of the augmented CNN. As it can be visualized in Fig.~\ref{fig:PCA-LCONV}, the two out-distribution sets, including CIFAR-100 (green triangles) and Fast Gradient Sign (FGS) adversaries~\citep{goodfellow2014explaining} (shown with yellow triangles) are separated from CIFAR-10 samples in the feature space of the augmented CNN while they are mixed in the feature space of its naive counterpart.






 


==> ICLR 2019 Out-distribution (6)/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

In this paper we bridge two issues of CNNs that were previously thought of as unrelated: susceptibility of naive CNNs to various types of adversarial examples and incorrect high confidence prediction for out-distribution samples. We argue these two issues are connected through over-generalization. We propose  augmented CNNs as a simple yet effective  solution for controlling over-generalization, when they are trained on an appropriate set of dustbin samples. Through empirical evidence, we define an indicator for selecting an ``appropriate'' natural out-distribution set as training samples for dustbin class from among those available and show such selection plays a vital role for training effective augmented CNNs. Through extensive experiments on several augmented CNNs in different settings, we demonstrate that reducing over-generalization can significantly reduce the misclassification error rates of CNNs on adversaries and out-distribution samples, simultaneously, while their accuracy rates on in-distribution samples are maintained. Indeed, reducing over-generalization by such an end-to-end learning model (e.g., augmented CNNs) leads to learning more expressive feature space where these two categories of hostile samples (i.e., adversaries and out-distribution samples) are disentangled from in-distribution samples. 



%In this paper we empirically demonstrate how CNNs augmented with out-distribution learning can either reject or correctly classify adversarial examples. Unlike previously proposed approaches our out-distribution learning approach does not rely on having access to adversarial examples which is useful as the approaches to generating such examples rapidly change and evolve. However, our approach is not foolproof and we we aim to assess our method with other attack models and on larger datasets. Also, we plan to assess our approach against white-box attacks and explore how it can be combined with other defenses to further reduce the error rate. 

==> ICLR 2019 Out-distribution (6)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\eg}{{\it e.g.,}\xspace}
\newcommand{\viz}{{\it viz.,}\xspace}
\newcommand{\Eg}{{\it E.g., }}
\newcommand{\etal}{{\it et~al.}}
\newcommand{\ie}{{\it i.e.,}\xspace}
\newcommand{\etc}{{\it etc.}}
\newcommand{\ci}{{\it (i) }}
\newcommand{\cii}{{\it (ii) }}
\newcommand{\ciii}{{\it (iii) }}
\newcommand{\civ}{{\it (iv) }}
\newcommand{\ca}{{\it (a) }}
\newcommand{\cb}{{\it (b) }}
\newcommand{\cc}{{\it (c) }}
\newcommand{\cd}{{\it (d) }}
\newcommand{\ce}{{\it (e) }}
\newcommand{\cf}{{\it (f) }}
\newcommand{\cg}{{\it (g) }}
\newcommand{\ch}{{\it (h) }}
%\newcommand{\ci}{{\it (i) }}
\newcommand{\cj}{{\it (j) }}
\newcommand{\ck}{{\it (k) }}
\newcommand{\cl}{{\it (l) }}
\newcommand{\cm}{{\it (m) }}
\newcommand{\cn}{{\it (n) }}
\newcommand{\co}{{\it (o) }}
\newcommand{\cp}{{\it (p) }}
\newcommand{\cq}{{\it (q) }}
%\newcommand{\note}{{\bf Note: }}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\eg}{{\it e.g.,}\xspace}
\newcommand{\viz}{{\it viz.,}\xspace}
\newcommand{\Eg}{{\it E.g., }}
\newcommand{\etal}{{\it et~al.}}
\newcommand{\ie}{{\it i.e.,}\xspace}
\newcommand{\etc}{{\it etc.}}
\newcommand{\ci}{{\it (i) }}
\newcommand{\cii}{{\it (ii) }}
\newcommand{\ciii}{{\it (iii) }}
\newcommand{\civ}{{\it (iv) }}
\newcommand{\ca}{{\it (a) }}
\newcommand{\cb}{{\it (b) }}
\newcommand{\cc}{{\it (c) }}
\newcommand{\cd}{{\it (d) }}
\newcommand{\ce}{{\it (e) }}
\newcommand{\cf}{{\it (f) }}
\newcommand{\cg}{{\it (g) }}
\newcommand{\ch}{{\it (h) }}
%\newcommand{\ci}{{\it (i) }}
\newcommand{\cj}{{\it (j) }}
\newcommand{\ck}{{\it (k) }}
\newcommand{\cl}{{\it (l) }}
\newcommand{\cm}{{\it (m) }}
\newcommand{\cn}{{\it (n) }}
\newcommand{\co}{{\it (o) }}
\newcommand{\cp}{{\it (p) }}
\newcommand{\cq}{{\it (q) }}
%\newcommand{\note}{{\bf Note: }}

